Type-Directed Program Synthesis for RESTful APIs

With the rise of software-as-a-service and microservice architectures, RESTful APIs are now ubiquitous in mobile and web applications. A service can have tens or hundreds of API methods, making it a challenge for programmers to find the right combination of methods to solve their task. We present APIphany, a component-based synthesizer for programs that compose calls to RESTful APIs. The main innovation behind APIphany is the use of precise semantic types, both to specify user intent and to direct the search. APIphany contributes three novel mechanisms to overcome challenges in adapting component-based synthesis to the REST domain: (1) a type inference algorithm for augmenting REST specifications with semantic types; (2) an efficient synthesis technique for "wrangling" semi-structured data, which is commonly required in working with RESTful APIs; and (3) a new form of simulated execution to avoid executing APIs calls during synthesis. We evaluate APIphany on three real-world APIs and 32 tasks extracted from GitHub repositories and StackOverflow. In our experiments, APIphany found correct solutions to 29 tasks, with 23 of them reported among top ten synthesis results.

==> fuzzing-graveyard.tex <==
% From overview

\mypara{Generating additional witnesses}
%
Mining accurate semantic types requires high-quality witnesses,
which exercise a rich set of API behaviors.
%
High-quality witnesses are hard to come by:
even open-source APIs rarely come with extensive test suites,
so for our experiments we obtained initial witnesses 
by manually driving a service through its Web UI. %, and recording browser traffic.
%
These witnesses often fail to exercise certain methods altogether,
therefore excluding them from type mining and synthesis.
%
To address this problem, 
\tool relies on the initial semantic type annotations 
to generate \emph{tests} for the service;
if successful, these tests produce additional witnesses,
resulting in mining more accurate types,
which in turn enables further test generation (see \autoref{fig:overview}).

For example, consider a different \sover question about the \slack API:
\emph{How to send a message to a user given their email?}
%
The idiomatic solution to this task requires calling \T{users.lookupByEmail},
which takes a user email and returns a user ID,
but is annotated as $\T{String} \to \T{String}$ in the spec.
%
Given only the initial witnesses in~\autoref{fig:witnesses},
\tool is unable to infer the semantic type of \T{users.lookupByEmail},
and hence to solve this task.
%
At the same time, generating useful tests for this method is challenging,
because it only succeeds on inputs that correspond to existing users' emails.
%
Instead of generating test inputs randomly,
\tool draws them from the bank of values it has observed in the existing witnesses;
in our example, one of the strings that appear in \autoref{fig:witnesses} is \T{"xyz@gmail.com"}.
%
Calling \T{users.lookupByEmail} with this string succeeds and returns \T{"UJ5RHEG4S"}.
%
Based on the previously mined types of these two strings,
\tool infers the type $\T{Profile.email} \to \T{User.id}$ for the new method.

%%% From Sec 4

\subsection{Augmenting Witnesses via Test Generation}\label{sec:mining:testing}

To infer precise semantic types for all methods in $\Lambda$,
\tool requires a large and versatile witness set $\witnesses$.
%
One way to obtain $\witnesses$ is by running an integration test suite;
unfortunately, for most proprietary services (including those used in our evaluation) 
such a test suite is not available.
%
Instead we collect witnesses by manually interacting with a service via its web interfaces
and recording web traffic.
%
Unfortunately, the set $\witnesses$ obtained this way is sparse,
which may prevent the mining algorithm from merging equivalent semantic types
or even inferring types for some methods altogether.
%
As an example, consider an initial witness set $\witnesses_0$,
which contains the three witnesses in \autoref{fig:witnesses}
together with the following witness for the method \T{users.profile.get},
whose syntactic type is $\{\T{user}:\T{String}\} \to \T{Profile}$:
\begin{equation}
  \langle \T{users.profile.get}, \{\T{user}=\T{"UITU592OF"}\}, \{\T{email}=\T{bat@inbox.com}, \T{display_name}=\T{"batman"}\} \rangle
\label{eq:profile-get}
\tag{$W_1$}
\end{equation}
%
Because the string \T{"UITU592OF"} appears nowhere else in $\witnesses_0$,
\tool has no way to infer that its semantic type is \T{User.id}.

To improve the quality and coverage of inferred types,
\tool generates additional witnesses,
using a combination of type-directed random testing and a small amount of manual annotations.
%
Continuing with our example,
recall that $\witnesses_0$ is sufficient to infer the semantic types in \autoref{tab:library}.
%
In particular, \tool knows that \T{conversations_members} takes as input a \T{Channel.id},
and hence can make more calls to this method using any channel ID in $\witnesses_0$
(in particular, IDs of other channels returned by \T{conversations_list}).
%
Assuming that one of the newly generated calls to \T{conversations_members} returns an array with \T{"UITU592OF"} in it,
running \textsc{MineTypes} with this new set of witnesses
will observe the same value at locations $\langle \T{users.profile.get}, \mathsf{in}.\T{user} \rangle$
and $\langle \T{conversations_members}, \mathsf{out}.\T{0} \rangle$,
and hence merge them into the same group, whose representative type is \T{User.id}.

\begin{figure}
  \centering
  \small
  \begin{algorithmic}[1]
      \Require{Library $\Lambda$, initial witnesses $\witnesses_0$}
      \Ensure{Semantic library $\sema{\Lambda}$}
      \Ensure{Augmented witnesses $\witnesses$}
      \Statex
      \Function{\textsc{AnalyzeAPI}}{$\Lambda, \witnesses_0$}
          \Let{$\witnesses$}{$\witnesses_0$}
          \Repeat
            \Let{$\sema{\Lambda}$}{\Call{MineTypes}{$\Lambda$, $\witnesses$}}
            \Let{$\witnesses$}{$\witnesses \cup \textsc{GenerateTests}(\sema{\Lambda})$}
          \Until{fixpoint or timeout}
          \State \Return{$\sema{\Lambda}, \witnesses$}
      \EndFunction
  \end{algorithmic}

  \centering
  \small
  \begin{algorithmic}[1]
      \Require{Semantic library $\sema{\Lambda}$}
      \Ensure{Generated witnesses $\witnesses$}
      \Statex
      \Function{\textsc{GenerateTests}}{$\sema{\Lambda}$}
        \For{$f\colon \{\many{l_i:\sema{t}_i}, \many{?l_j:\sema{t}_j}\} \to \sema{t}_o \in \sema{\Lambda}$}
          \Let{$\sema{t}_{req}, \sema{t}_{opt}$}{$\{\many{l_i:\sema{t}_i}\}, \{\many{?l_j:\sema{t}_j}\}$}
          \For{$\sema{t}_{sub} \subset \sema{t}_{opt}$}
            \Let{$v_{in}$}{$\{ \}$}
            \For{$l:\sema{t} \in \sema{t}_{req}\cup\sema{t}_{sub}$}
              \Let{$v_{in}.l$}{$\mathsf{random}(\sema{\Lambda}.\bank[\sema{t}])$}              
            \EndFor
            \Let{$v_{out}$}{$\mathsf{call}(f, v_{in})$}
            % \If{$v_{out} \neq \bot$}
            \State{\textbf{if} $v_{out} \neq \bot$ \textbf{then} \textbf{yield} $\langle f, v_{in}, v_{out} \rangle$}
            % \EndIf
          \EndFor
        \EndFor
      \EndFunction
  \end{algorithmic}
  \caption{Top-level API analysis algorithm and test generation.}
  \label{alg:analyze}
\end{figure}


The top-level API analysis algorithm of \tool is depicted in \autoref{alg:analyze} (left).
%
The algorithm alternates between calls to \textsc{MineTypes}
(to compute the best semantic library $\sema{\Lambda}$ it can mine from the current witnesses $\witnesses$)
and \text{GenerateTests}
(to augment $\witnesses$ using the current $\sema{\Lambda}$).
%
Analysis terminates either if $\sema{\Lambda}$ and $\witnesses$ reach a fixpoint,
or when a timeout is reached.
%
The algorithm returns both $\sema{\Lambda}$, which is used to build the TTN during the synthesis step,
and $\witnesses$, which is used for retrospective execution during the ranking step;
hence augmenting $\witnesses$ also improves the quality of ranking.
% (in addition to improving $\sema{\Lambda}$).

\mypara{Type-driven test generation}
%
\autoref{alg:analyze} (right) presents the algorithm \textsc{GenerateTests},
which generates new witnesses via random testing.
%
Note that this algorithm is written as a co-routine,
\ie it yields one witness at a time
(our implementation instead yield witnesses in batches).
%
At a high level, \textsc{GenerateTests} iterates through the method signatures in $\sema{\Lambda}$,
and for every method $f\colon \sema{t}_i \to \sema{t}_o$,
it samples a random input of type $\sema{t}_i$,
makes an API call to $f$ with that input,
and if the call succeeds, yields the corresponding witness.

How does \tool generate random inputs of a given semantic type,
such as \T{User.id}?
%
To this end, we augment the semantic library $\sema{\Lambda}$
with a \emph{value bank} $\bank$,
which is a mapping from semantic types to sets of values.
%
The value bank gets populated during type mining
(more specifically during the \textsc{Flatten} step in \autoref{fig:comp-inference}),
and contains all values that appear in $\witnesses$;
for arrays and objects, it also contains their constituents. 
%
For example, after processing the first witness in \autoref{fig:witnesses},
$\bank$ contains, among others, the entries $\T{Channel} \mapsto \lbrace \{\ \T{id} = \T{"C12345678"}, \T{creator} = \T{"UJ5RHEG4S"}, \ldots \}, \ldots \rbrace$,
$\T{Channel.id} \mapsto \lbrace \T{"C12345678"}, \ldots \rbrace $, 
and $\T{Channel.creator} \mapsto \lbrace \T{"UJ5RHEG4S"}, \ldots \rbrace$. 
%
During mining, when different semantic types are merged, their bank entries are also merged;
for example $\bank[\T{Channel.creator}]$ is later merged into $\bank[\T{User.id}]$.
%
% For example, when \T{Channel.creator} and \T{User.id} are merged 
% (and the latter is chosen as the representative),
% all values from $\bank[\T{Channel.creator}]$ are merged into $\bank[\T{User.id}]$
% and the former entry is removed from the bank.
%
\textsc{GenerateTests} uses the value bank (denoted $\sema{\Lambda}.\bank$) at line 7
to randomly sample an input from all values stored at semantic type $\sema{t}$.

With the value bank at hand,
generating tests is otherwise relatively straightforward.
%
The only complication arises because many API methods have optional arguments
and behave differently depending on which subset of optional arguments is provided.
%
To cover a wide range of method behaviors,
\textsc{GenerateTests} partitions the record of all arguments $\sema{t}_i$
into two records, each containing either only required or only optional arguments (line 3).
%
The algorithm then iterates over all subsets of optional arguments (line 4),
attempting to make a call for each subset
(our implementation only iterates over subsets up to a pre-defined size).

\mypara{Manual annotations}
%
Fully automatic test generation helps us bootstrap semantic type inference
for methods that already appear in $\witnesses_0$,
but it unfortunately cannot add witnesses for methods that are missing entirely.
%
For example, consider a $\witnesses_0$
that includes only the three witnesses in \autoref{fig:witnesses},
and does \emph{not} include the witness \eqref{eq:profile-get} for \T{users.profile.get}.
%
Because \tool has not seen any examples of input strings for this method,
no amount of witnesses for other methods would enable it to infer the semantic input type for \T{users.profile.get},
since there are no values it can merge.

To address this problem, a natural idea is to try one value for each semantic type
so that we are able to figure out which semantic type makes the call succeed.
%
% Aside from the problem that a value with the correct semantic type may fail a method call,
The main obstacle for us to adopt this approach is that
in the worst case, we would have to make a prohibitively large number of method calls.
%
Suppose we have $n$ semantic types and $k$ arguments for an unknown method;
this approach would require us to try $O(n^k)$ method calls to guess the semantic types for all arguments.
%
Instead of doing this, we manually add consumer-producer annotations 
to those methods missing from $\witnesses_0$.
%
For example, for \T{users.profile.get},
we add an annotation specifying that its input can be generated
by invoking \T{conversations_members}
and accessing any element of its response array.
%
Our evaluation (\autoref{sec:eval}) shows
that a modest amount of manual annotations
combined with type-directed test generation
enables \tool to obtain good coverage of real-world APIs.



